A Lower Bound of the Number of Rewrite Rules Obtained by Homological Methods

It is well-known that some equational theories such as groups or boolean algebras can be defined by fewer equational axioms than the original axioms. However, it is not easy to determine if a given set of axioms is the smallest or not. Malbos and Mimram investigated a general method to find a lower bound of the cardinality of the set of equational axioms (or rewrite rules) that is equivalent to a given equational theory (or term rewriting systems), using homological algebra. Their method is an analog of Squier's homology theory on string rewriting systems. In this paper, we develop the homology theory for term rewriting systems more and provide a better lower bound under a stronger notion of equivalence than their equivalence. The author also implemented a program to compute the lower bounds, and experimented with 64 complete TRSs.

==> equivalences.tex <==
Let $\Sigma$ be a signature.
Two TRSs $(\Sigma,R_1)$ and $(\Sigma,R_2)$ are said equivalent if $\xleftrightarrow{*}_{R_1}\,=\,\xleftrightarrow{*}_{R_2}$.
In this section, we consider a notion of ``equivalence'' between TRSs $(\Sigma_1,R_1)$ and $(\Sigma_2,R_2)$ where $\Sigma_1$ and $\Sigma_2$ can be different.

For $t \in T(\Sigma)$ with variables $x_1,\dotsc,x_n$ and $t_1,\dotsc,t_n \in T(\Sigma)$, let $t[t_1/x_1,\dotsc,t_n/x_n]$ denote the term obtained by substituting $t_i$ for $x_i$ in $t$ for each $i=1,\dotsc,n$ in parallel.
For example, $f(x_1,x_2)[g(x_2)/x_1,g(x_1)/x_2] = f(g(x_2),g(x_1))$.
\begin{definition}
For two TRSs $(\Sigma_1,R_1)$, $(\Sigma_2,R_2)$ are Tietze equivalent if there is a map $F : T(\Sigma_1) \rightarrow T(\Sigma_2)$ satisfying
\begin{enumerate}
  \item $F(x) = x$ for any variable $x$, \label{Teqvar}
  \item $F(f(t_1,\dotsc,t_n)) = F(f(x_1,\dotsc,x_n))[F(t_1)/x_1,\dotsc,F(t_n)/x_n]$ for $f \in \Sigma$ with arity $n$, \label{Teqsym}
  \item Let $T_k(\Sigma)$ be the set of terms in $T(\Sigma)$ whose variables are in $\{x_1,\dots,x_k\}$, and let $\sim_{i,k}$ be $\xleftrightarrow{*}_{R_i}|_{T_k(\Sigma)\times T_k(\Sigma)}$, the restriction of $\xleftrightarrow{*}_{R_i}$ to $T_k(\Sigma)\times T_k(\Sigma)$.
  Then, $F$ induces the bijection $\tilde F_k : (T_k(\Sigma_1)\quot\sim_{1,k}) \rightarrow (T_k(\Sigma_2)\quot\sim_{2,k})$ for each $k$, i.e., the map $\tilde F_k([t]_1) := [F(t)]_2$ $(t \in T_k(\Sigma_1))$ is well-defined and bijective where $[t]_{i}$ is the equivalence class of $t$ by $\sim_{i,k}$. \label{Teqbij}
\end{enumerate}
\end{definition}
This definition of Tietze equivalence is taken from \cite{mm16}, but stated in a way without category theoretic terminology.
Notice that the map $F : T(\Sigma_1)\rightarrow T(\Sigma_2)$ that satisfies \ref{Teqvar} and \ref{Teqsym} is uniquely determined if the value of $F$ of $f(x_1,\dotsc,x_n)$ is given for every $f^{(n)}\in\Sigma_1$.
Also notice that the condition \ref{Teqbij} implies $t \xleftrightarrow{*}_{R_1} s \iff F(t) \xleftrightarrow{*}_{R_2} F(s)$.
It is obvious that any equivalent TRSs $(\Sigma,R_1)$,$(\Sigma,R_2)$ are Tietze equivalent since the map $F(t) = t$ ($t \in T(\Sigma)$) satisfies the three conditions above.
We have an operational characterization of Tietze equivalence:
\begin{proposition}
  Two TRSs $(\Sigma_1,R_1)$, $(\Sigma_2,R_2)$ are Tietze equivalent if and only if $(\Sigma_1,R_1)$ and $(\Sigma_2,R_2)$ are transformed to each other by the sequence of the following four operations:
  \begin{description}
    \item[T1. Adding a superfluous symbol]
    \[
      (\Sigma,R) \mapsto (\Sigma\uplus\{f\},R\uplus\{t\rrule f(x_1,\dotsc,x_n)\}),
    \]
where $f\notin\Sigma$ is an $n$-ary symbol and $t$ is a term in $T(\Sigma)$ whose variables are in $\{x_1,\dotsc,x_n\}$,
    \item[T1'. Removing a superfluous symbol]
    \[
      (\Sigma,R) \mapsto (\Sigma\setminus\{f\}, R\setminus\{t\rrule f(x_1,\dotsc,x_n)\}),
      \]
where $f\in \Sigma$ is an $n$-ary symbol, $t$ is a term in $T(\Sigma)$ whose variables are in $\{x_1,\dots,x_n\}$, and $t\rrule f(x_1,\dotsc,x_n)$ is the only element in $R$ which involves $f$,
    \item[T2. Adding a derivable relation]
    \[
      (\Sigma,R) \mapsto (\Sigma,R\cup\{t\rrule s\})
    \]
where $t,s\in T(\Sigma)$ satisfy $t\rewrst{R}s$,
    \item[T2'. Removing a derivable relation]
    \[
      (\Sigma,R) \mapsto (\Sigma,R\setminus\{t\rrule s\})
    \]
where $t,s \in T(\Sigma)$ satisfy $t\rewrst{R} s$.
  \end{description}
\end{proposition}
These four operations are called \textit{Tietze transformations} \cite{mm16}.
Tietze equivalence is originally introduced in group theory \cite[\S 11]{t1908}
and is also defined for monoids \cite[7.2]{bo93}.

\begin{example}
  Consider the signature $\Sigma = \{+^{(2)},S^{(1)},0^{(0)}\}$ and the set $R$ of four rules
  \[
    0 + x \rrule x,\ x + 0 \rrule x,\ S(x) + y\rrule S(x + y),\ (x + y) + z \rrule x + (y + z).
  \]
  We can see $(\Sigma,R)$ is Tietze equivalent to $(\Sigma',R')$ where
  \[
   \Sigma' = \{+^{(2)},0^{(0)},1^{(0)}\},\ R' = \{0 + x \rrule x,\ x + 0 \rrule x,\ (x + y) + z \rrule x + (y + z)\}
   \]
   as follows:
   \begin{align*}
     (\Sigma,R)
     &\xlongrightarrow{\rm T1} (\Sigma\uplus \{1^{(0)}\}, R\uplus\{S(0) \rrule 1\})\\
     &\xlongrightarrow{\rm T2} (\Sigma\uplus\{1^{(0)}\}, R\uplus\{S(0) \rrule 1,\ 1 + x\rrule S(x)\})\\
     &\xlongrightarrow{\rm T2'} (\Sigma\uplus\{1^{(0)}\}, R\uplus\{1+x\rrule S(x)\})\\
     &\xlongrightarrow{\rm T2'} (\Sigma\uplus\{1^{(0)}\}, R\uplus\{1+x\rrule S(x)\}\setminus\{S(x)+y\rrule S(x+y)\})\\
     &\xlongrightarrow{\rm T1'} (\Sigma\uplus\{1^{(0)}\}\setminus\{S^{(1)}\}, R\setminus\{S(x)+y\rrule S(x+y)\})
     = (\Sigma',R').
   \end{align*}
\end{example}
\begin{example}
Boolean algebra is presented by $\Sigma = \{\land^{(2)},\lor^{(2)},\lnot^{(1)},\top^{(0)},\bot^{(0)}\}$ and set $R$ of rules
\[
\begin{array}{rlrl}
  x_1\land x_1 &\rrule x_1,& x_1\lor x_1 &\rrule x_1,\\
  x_1 \land x_2 &\rrule x_2 \land x_1,&  x_1 \lor x_2 &\rrule x_2 \lor x_1,\\
  (x_1 \land x_2) \land x_3 &\rrule x_1 \land (x_2 \land x_3),&
  (x_1 \lor x_2) \lor x_3 &\rrule x_1 \lor (x_2 \lor x_3),\\
  (x_1 \land x_2) \lor x_1 &\rrule x_1& (x_1 \lor x_2)\land x_1 &\rrule x_1,\\
  (x_1 \land x_2) \lor x_3 &\rrule (x_1 \lor x_3) \land (x_2 \lor x_3),&
  (x_1 \lor x_2) \land x_3 &\rrule (x_1 \land x_3) \lor (x_2 \land x_3),\\
  x_1\land \lnot x_1 &\rrule \bot,& x_1 \lor \lnot x_1 &\rrule \top.
\end{array}
\]
Since we have rule $x_1\land \lnot x_1 \rrule \bot$, one may want to remove symbol $\bot$ by the operation T1'.
However, this is not allowed because term $x_1\land\lnot x_1$ has more variables than term $\bot$.
(Recall that adding/removing symbol $f$ and rule $t\rrule f(x_1,\dotsc,x_n)$ by T1/T1' requires the variables of $t$ are involved in $\{x_1,\dotsc,x_n\}$.)
Indeed, we can prove
$(\Sigma',R')=(\Sigma\setminus\{\bot\},R\setminus\{x_1\land\lnot x_1\rrule \bot\})$
is not Tietze equivalent to $(\Sigma,R)$ with map
$F:T(\Sigma')\ni t \mapsto t\in T(\Sigma)$:
since
\[
\sim_0 := \rewrst{R}|_{T_0(\Sigma)\times T_0(\Sigma)}=\{(\top,\top)\}
\]
 and
\[
\sim'_0:=\rewrst{R'}|_{T_0(\Sigma')\times T_0(\Sigma')}=\{(\bot,\bot),(\top,\top)\},
\]
we have
$T_0(\Sigma)\quot\sim_0 \ = T_0(\Sigma) = \{\bot,\top\}$,
$T_0(\Sigma')\quot\sim'_0 \ = \ T_0(\Sigma') = \{\top\}$,
so $\tilde F_0 : (T_0(\Sigma)\quot\sim_0) \rightarrow (T_0(\Sigma')\quot\sim'_0)$ is not a bijection.
We can show the same thing for $\top$ and $x_1\lor\lnot x_1\rrule \top$.
It is also valuable to study \textit{equivalence} in the sense that allows to remove $\bot$ and $\top$,
and certainly some researchers study equivalent axiom sets of Boolean algebra in that sense \cite{h33,m02}.
However, such axiom sets without $\bot$ and $\top$ have the empty set as their model,
on the other hand the original definition of Boolean algebra requires the existence of elements $\bot$ and $\top$.
\end{example}


==> inefficient.tex <==
\label{section:inefficient}
We construct and prove that there exists an inefficient TRS.

Let us consider the signature $\Sigma = \{a_1^{(1)},a_2^{(1)},a_3^{(1)},b^{(1)}\}$ and the set $R$ of rewrite rules
\begin{align*}
    a_i^7(x) &\rightarrow x \quad (i=1,2,3)\\
    a_i(a_j(x)) &\rightarrow a_j(a_i(x)) \quad (j < i, i=2,3, j = 1,2)\\
    b^3(x) &\rightarrow x\\
    b(a_i(x)) &\rightarrow a_i^2(b(x)) \quad (i=1,2,3)
\end{align*}
\begin{defi}
Let $(\Sigma,R)$ be a TRS.
\begin{enumerate}
\item $(\Sigma,R)$ is a \emph{groupoid} if for any bicontext $(C,t)$ 
\item A \emph{sub-TRS} of $(\Sigma,R)$ is a TRS satisfying
$t \xleftrightarrow[R']{*} s \iff t \xleftrightarrow[R]{*} s$
for any $t,s\in T(\Sigma')$.
\item a \emph{subgroupoid} of $(\Sigma,R)$ if $(\Sigma',R')$ is a sub-TRS of $(\Sigma,R)$ and for any 
\end{enumerate}
\end{defi}
Suppose $A'=(\Sigma',R')$ is a sub-TRS of $A=(\Sigma,R)$.
Let $[(C,t)]\in \overline{\imonring{\bbK}}^{A}(i,j)$ be a coset of bicontext.
We write $A'[(C,t)](k)$ for the set
\[
\{[(D,s)\circ(C,t)]\mid (D,s)\in\overline{\imonring{\bbK}}^{A'}(j,k)\}
\]
and $\lcoset{A'}{A}(i,k)$ for
\[
\{A'[(C,t)](k)\mid (C,t)\in\overline{\imonring{\bbK}}^{A}(i,j),\ j \in \bbN\}.
\]
Note that $A'[(C,t)](k)$ and $A'[(D,s)](k)$ can be the same set for different $(C,t)$ and $(D,s)$.
Therefore, even if each $\overline{\imonring{\bbK}}^{A}(i,j)$ contains infinitely many cosets of bicontext, $\lcoset{A'}{A}(i,k)$ can be a finite set.
\begin{defi}
Suppose $A'=(\Sigma',R')$ is a sub-TRS of $(\Sigma,R)$.
The $(i,k)$-\emph{index} of $A'$ in $A$ is the cardinality of the set $\lcoset{A'}{A}(i,k)$, denoted by $\gindex{A}{A'}(i,k)$.
\end{defi}
The set $A'[(C,t)](k)$ is an analog of the ``right coset'' in group theory and the $(i,k)$-index corresponds to the index of a subgroup.

Let $A'=(\Sigma',R')$ be a sub-TRS of a TRS $A=(\Sigma,R)$,
$\Gamma_{i,j}$ be a finite set for each $i = 0,1,2,\ j\in \bbN$,
and $\Gamma_i$ be $\{\Gamma_{i,0},\Gamma_{i,1},\Gamma_{i,2},\dots\}$.
For each $a\in \lcoset{A'}{A}(i,j)$, we choose $[(C_a,t_a)] \in \cR^A(i,j)$ such that $A'[(C_a,t_a)](j) = a$.
We define $\Gamma'_{i,j} = \{(a,p)\mid a\in \lcoset{A'}{A}(i,j), p \in \Gamma_{i,j}\}$ and $\Gamma'_i = \{\Gamma'_{i,0},\Gamma'_{i,1},\Gamma'_{i,2},\dots\}$.
Since any $[(D,s)]\in \cR^A(i,j)$ is equal to $[(D',s')\circ (C_a,t_a)]$ for a unique $a\in \lcoset{A'}{A}(i,j)$,
the following $\cR^{A'}$-linear map $\freemod{\cR^A}{\Gamma_i}\rightarrow \freemod{\cR^{A'}}{\Gamma'_i}$ is well-defined:
\[
\phi_i([(D,s)]\underline{p}) = [(D',s')]\underline{([(C_a,t_a)],p)} \quad ([(D,s)]=[(D',s')\circ(C_a,t_a)]).
\]
We can check $\phi_i$ has its inverse
\[
\phi_i^{-1}([(D',s')]\underline{([(C_a,t_a)])}) = [(D',s')\circ(C_a,t_a)]\underline{p} = [(D,s)]\underline{p}.
\]
\begin{prop}
In the setting of the above paragraph, if the sequence of free left $\cR^A$-modules
\[
\freemod{\cR^A}{\Gamma_2} \xrightarrow{\partial_2}
\freemod{\cR^A}{\Gamma_1} \xrightarrow{\partial_1}
\freemod{\cR^A}{\Gamma_0} \xrightarrow{\epsilon}
\cZ \rightarrow 0
\]
is exact, then
\[
\freemod{\cR^{A'}}{\Gamma'_2} \xrightarrow{\partial'_2}
\freemod{\cR^{A'}}{\Gamma'_1} \xrightarrow{\partial'_1}
\freemod{\cR^{A'}}{\Gamma'_0} \xrightarrow{\epsilon'}
\cZ \rightarrow 0
\]
is also exact where $\partial'_i = \phi_i\circ \partial_i \circ \phi_i^{-1}$ for $i=1,2$ and $\epsilon'_i = \phi_i\circ \epsilon_i\circ \phi_i^{-1}$.
\end{prop}
\begin{proof}
By definition,
$\partial_1'\circ \partial_2' = 0$,
$\epsilon' \circ \partial'_1 = 0$
follows from
$\partial_1 \circ \partial_2 = 0$,
$\epsilon \circ \partial_1 = 0$.
If $[(D,s)]\underline{(a,p)})\in \ker \partial'_1$,
then $\partial'_1([(D,s)]\underline{(a,p)})=\phi_1\circ\partial_1([(D,s)\circ(C_a,t_a)]\underline{p})=0$, so we have
$\partial_1([(D,s)\circ(C_a,t_a)]\underline{p})=0$,
or equivalently, $[(D,s)\circ(C_a,t_a)]\underline{p} \in \ker\partial_1$.
Therefore
$[(D,s)\circ(C_a,t_a)]\underline{p}\in \im \partial_2$, \ie,
there exists $[(E,u)]\underline{q} \in \freemod{\cR^A}{\Gamma_2}$ such that
$\partial_2([(E,u)]\underline{q})=[(D,s)]\circ[(C_a,t_a)]\underline{p}$.

\end{proof}
\begin{defi}
Let $(\Sigma,R)$ be a TRS.
Suppose $F_\bullet$ is a partial resolution
\[
F_2 \rightarrow F_1 \rightarrow F_0 \rightarrow \cZ \rightarrow 0
\]
of $\cR$ over $\cR$.
\[
\mu(F_\bullet) = f_2 - f_1 + f_0 
\]
\end{defi}
